Radio identification of decametric sources. I. Catalogue

We describe a method of plotting continuous spectra for radio sources on the basis of entries of various source catalogues in comparatively large error boxes around a given sky position. Sources from the UTR-2 catalogue (Braude et al., 1978, 1979, 1981, 1985, 1994), observed at decametric wavelengths (10--25 MHz) with an antenna beam of about 40', were cross-identified with entries from other radio catalogues at higher frequencies. Using the CATS database we extracted all sources within 40' around UTR positions to find candidate identifications. The spectrum for each source was fitted with a set of curves using the least squares method to find the best fit. We preferentially selected radio counterparts whose radio spectrum extrapolated to low frequencies matched the UTR decametric flux densities, and whose coordinates were close to the gravity centre of UTR positions. Among all 1822 sources in the UTR catalogue we found about 350 sources to be blends of two or more sources. As the most probable true coordinates of the radio counterparts we used positions from the FIRST, NVSS, TXS, GB6, or PMN catalogues. Using low-frequency sources (26, 38, 85 MHz) from CATS we checked the reliability of some of our identifications. We show examples `of the above methods, including raw and ``cleaned'' spectra. Identifications with objects from optical, X-ray and infrared catalogues, as well as a subsample of UTR sources with ultra-steep spectrum are presented.

==> landpage.tex <==
% *** Layout for landscape A4 (v.1.0)
% *** for article.sty, sao1.sty, sao2.sty
%

\newlength{\tmptextheight}
\setlength{\tmptextheight}{\textheight}
\newlength{\tmpoddsidemargin}
\setlength{\tmpoddsidemargin}{\oddsidemargin}

%\oddsidemargin= -2.5mm   % handling
%\evensidemargin= -2.5mm  % handling

% Calculation of \odd... and \evensidemargin
\oddsidemargin=848.6pt                 % size of A4 (297mm)
\advance\oddsidemargin by -72.6pt      % 1in(25.4mm)
\advance\oddsidemargin by -\topmargin
\advance\oddsidemargin by -\headheight
\advance\oddsidemargin by -\headsep
\advance\oddsidemargin by -\textheight
\advance\oddsidemargin by -72.6pt      % 1in(25.4mm)
%\advance\oddsidemargin by -\footskip  % add for {article}
\evensidemargin=\oddsidemargin

%\textheight=\textwidth      % for tabular
\textheight=1.1\textwidth   % add for supertabular 10%
\textwidth=\tmptextheight
\headheight=0pt
\headsep=0pt
\topmargin=\tmpoddsidemargin

